Demographic parity in regression and classification within the unawareness framework

This paper explores the theoretical foundations of fair regression under the constraint of demographic parity within the unawareness framework, where disparate treatment is prohibited, extending existing results where such treatment is permitted. Specifically, we aim to characterize the optimal fair regression function when minimizing the quadratic loss. Our results reveal that this function is given by the solution to a barycenter problem with optimal transport costs. Additionally, we study the connection between optimal fair cost-sensitive classification, and optimal fair regression. We demonstrate that nestedness of the decision sets of the classifiers is both necessary and sufficient to establish a form of equivalence between classification and regression. Under this nestedness assumption, the optimal classifiers can be derived by applying thresholds to the optimal fair regression function; conversely, the optimal fair regression function is characterized by the family of cost-sensitive classifiers.

==> biblio.tex <==
Research on optimal prediction under demographic constraint has primarily focused on classification, where the goal is to predict a binary response in $\{0,1\}$, as this problem is intrinsically linked to the central issue of fair candidate selection in algorithmic fairness. This problem is well understood in the awareness setting from an algorithmic point of view \citep{Feldman15,pmlr-v81-menon18a,NEURIPS2020_29c0605a, pmlr-v161-schreuder21a,NEURIPS2022_b1d9c7e7,JMLR:v25:23-0322}. On the theoretical side, \cite{pmlr-v206-gaucher23a} proved recently that the optimal classifier can be obtained as the indicator that the optimal fair prediction function for the squared loss is above a given threshold, as result then extended in \cite{pmlr-v202-xian23b} to multi-class classification. 

By contrast, less is known for fair classification in the unwareness framework. On the algorithmic side, a body of work considers linear classifiers, and proposes various relaxations of the demographic parity constraint leading to tractable algorithms for calculating the classifier \citep{NIPS2016_dc4c44f6, JMLR:v20:18-262}. On the theoretical side, \cite{liptonDisparity} provide empirical evidence suggesting that fair classifiers may base their decisions on non-relevant features correlated with the sensitive attribute, potentially disrupting within-group ordering.  This hypothesis was further confirmed by \cite{pmlr-v206-gaucher23a}, who characterized the optimal fair classifier without disparate treatment. They showed that it is given by the indicator that the conditional expectation $\eta(X)$ is above a threshold, which depends on the probabilities that the individual described by $X$ belongs to the different groups. In particular, the question of whether this classifier can be reformulated as the indicator function that the optimal fair prediction function for the squared loss without disparate treatment is above a given threshold remains unresolved.

The problem of fair regression within the unawareness framework has been seldom studied, particularly from a theoretical perspective. One reason is that the demographic parity constraint is harder to implement without disparate treatment. Algorithms complying with these constraints have been proposed by \cite{Chzhen2020AnEO} and \cite{zhou2023groupblind}, but the authors do not claim that the estimators obtained are optimal in terms of risk. \cite{pmlr-v97-agarwal19d} propose an algorithm based on a discretization of the problem, followed by a reduction to cost-sensitive classification. However, their algorithm requires calling an oracle cost-sensitive classifier, which may not be computable. Moreover, their results hold for a class of regression functions with bounded Rademacher complexity. In this paper, we focus on the theoretical aspects of this problem, specifically on characterizing and studying the optimal regression function.
